Ultrasonic imaging in highly heterogeneous backgrounds

This work formally investigates the differential evolution indicators as a tool for ultrasonic tracking of elastic transformation and fracturing in randomly heterogeneous solids. Within the framework of periodic sensing, it is assumed that the background contains (i) a multiply connected set of viscoelastic, anisotropic, and piecewise homogeneous inclusions, and (ii) a union of possibly disjoint fractures and pores. The support, material properties, and interfacial condition of scatterers in (i) and (ii) are unknown, while elastic constants of the matrix are provided. The domain undergoes progressive variations of arbitrary chemo-mechanical origins such that its geometric configuration and elastic properties at future times are distinct. At every sensing step $t_\circ, t_1, \ldots,$ multi-modal incidents are generated by a set of boundary excitations, and the resulting scattered fields are captured over the observation surface. The test data are then used to construct a sequence of wavefront densities by solving the spectral scattering equation. The incident fields affiliated with distinct pairs of obtained wavefronts are analyzed over the stationary and evolving scatterers for a suit of geometric and elastic evolution scenarios entailing both interfacial and volumetric transformations. The main theorem establishes the invariance of pertinent incident fields at the loci of static fractures and inclusions between a given pair of time steps, while certifying variation of the same fields over the modified regions. These results furnish a basis for theoretical justification of differential evolution indicators for imaging in complex composites which, in turn, enable the exclusive tomography of evolution in a background endowed with many unknown features.

==> ArXiv submission/macros.tex <==
%%%\
%%%   Macros (mostly for mathematical formulas)
%%%
\newlength{\kaka}
\newcommand{\dd}[1]{\protect\settowidth{\kaka}{\mbox{$#1$}}\makebox[\kaka]{$\buildrel{\scriptscriptstyle}\over{#1}$}}
\newcommand{\ahref}[2]{}
\newcommand{\der}[2]{\frac{d#1}{d#2}}
\newcommand{\Tsup}{^{\text{\tiny T}}}
\newcommand{\Rsub}{_{\text{\tiny R}}}
\newcommand{\Isub}{_{\text{\tiny I}}}
\newcommand{\Isup}{^{\text{\tiny I}}}
\newcommand{\Esup}{^{\text{\tiny E}}}
\newcommand{\Zsup}{^{\text{\tiny o}}}
\newcommand{\Zsub}{_{\text{\tiny o}}}
\newcommand{\zsub}{_{\!\text{\tiny o}}}
\newcommand{\hard}{_{\text{hard}}}
\newcommand{\soft}{_{\text{soft}}}
\newcommand{\obs}{^{\text{obs}}}
\newcommand{\opt}{_{\text{\tiny{opt}}}}
\newcommand{\true}{^{\text{\tiny true}}}
\newcommand{\eps}{\epsilon}
\newcommand{\px} {\accentset{\star}{p}}
\newcommand{\fx} {\accentset{\star}{f}}
\newcommand{\gx} {\accentset{\star}{g}}

\newcommand{\Sf}{S^{\text{\tiny f}}}
\newcommand{\Sb}{S^{\text{\tiny b}}}
\newcommand{\Lf}{L^{\text{\tiny f}}}
\newcommand{\ff}{^{\text{\tiny f}}}

\newcommand{\one}{_{\text{\tiny I}}}
\newcommand{\two}{_{\text{\tiny I\nxs I}}}

\newcommand{\jed}{{\text{I}}}
\newcommand{\dva}{{\text{I\nxs I}}}

\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\rhoo}{\uprho_{\circ}}
\newcommand{\muo}{\upmu_{\circ}}
\newcommand{\lambdao}{\uplambda_{\circ}}

\newcommand\eqvar{\stackrel{\alpha}{=}}
\newcommand\eqvarm[1]{\stackrel{\alpha^{#1}}{=}}

\newcommand{\lcba}{\left\{\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rcba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right\}} 

\newcommand{\lsba}{\left(\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rsba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right)}

\newcommand{\lcbc}{\left\{\rule{0cm}{0.35cm}\hspace{-0.1cm}\right.}
\newcommand{\rcbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.35cm}\right\}}

\newcommand{\lsqba}{\left[\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rsqba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right]}

\newcommand{\lsqbc}{\left[\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rsqbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right]}

\newcommand{\lsbc}{\left(\rule{0cm}{0.35cm}\hspace{-0.1cm}\right.}
\newcommand{\rsbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.35cm}\right)}

\newcommand{\lsbb}{\left(\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rsbb}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right)}

\newcommand{\lqbb}{\left[\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rqbb}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right]}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\lb}{\label}
\newcommand{\nn}{\nonumber}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bxr}{\begin{array}}
\newcommand{\exr}{\end{array}}

\newcommand\exs{\hspace*{0.4mm}}
\newcommand\xxs{\hspace*{0.2mm}}
\newcommand\nes{\hspace*{-0.4mm}}
\newcommand\nxs{\hspace*{-0.2mm}}
\newcommand\nms{\hspace*{-0.3mm}}

\newenvironment{proof57}{\paragraph*{Proof of Theorem 5.7.}}{\hfill$\blacksquare$}
\newenvironment{proof59}{\paragraph*{Proof of Theorem 5.9.}}{\hfill$\blacksquare$}

\def\asym{\mathop{\rm Asym}}
\newcommand{\abs}[1]{\left| #1 \right|}  
\newcommand{\norms}[1]{\parallel\! #1 \!\parallel} 
\newcommand{\inv}[1]{\frac{1}{#1}}
\newcommand{\nnum}{\notag \\}
\newcommand{\suite }{\nnum & \mbox{}\hspace{15pt}}
\newcommand{\bfna}{\nabla}
\newcommand{\demi} {\inv{2}}
\newcommand{\bfG} {\boldsymbol{G}}
\newcommand{\bA} {\boldsymbol{A}}
\newcommand{\bU} {\boldsymbol{U}}
\newcommand{\bSig} {\boldsymbol{\Sigma}}
\newcommand{\bW} {\boldsymbol{W}}
\newcommand{\bC} {\boldsymbol{C}}
\newcommand{\bK} {\boldsymbol{K}}
\newcommand{\bV} {\boldsymbol{V}}
\newcommand{\bR} {\boldsymbol{\sf R}}
\newcommand{\bJ} {\boldsymbol{J}}
\newcommand{\bM} {\boldsymbol{M}}
\newcommand{\bQ} {\boldsymbol{Q}}
\newcommand{\bH} {\boldsymbol{H}}
\newcommand{\btau} {\boldsymbol{\tau}}
\newcommand{\bn} {\boldsymbol{n}}
\newcommand{\ba} {\boldsymbol{a}}
\newcommand{\bb} {\boldsymbol{b}}
\newcommand{\bfn} {\boldsymbol{n}}
\newcommand{\bfP} {\boldsymbol{P}}
\newcommand{\bfPt} {\dd{\bfP}}
\newcommand{\bfp} {\boldsymbol{p}}
\newcommand{\bfe} {\boldsymbol{e}}
\newcommand{\bfw} {w}
\newcommand{\bx} {\boldsymbol{x}}
\newcommand{\by} {\boldsymbol{y}}
\newcommand{\be} {\boldsymbol{e}}
\newcommand{\bh} {\boldsymbol{h}}
\newcommand{\bz} {\boldsymbol{z}}
\newcommand{\bg} {{\boldsymbol{g}}}
\newcommand{\bq} {{\boldsymbol{q}}}
\newcommand{\bgt} {\tilde{\bg}}
\newcommand{\ii} {\textrm{i}}
\newcommand{\oG} {\overline{G}}
\newcommand{\bxb} {\bar{\boldsymbol{x}}}
\newcommand{\bm} {\boldsymbol{m}}
\newcommand{\bfx} {\boldsymbol{x}}
\newcommand{\bfX} {\boldsymbol{X}}
\newcommand{\bfXt} {\dd{\bfX}}
\newcommand{\bft} {\boldsymbol{t}}
\newcommand{\bfT} {\boldsymbol{T}}
\newcommand{\bfTt} {\tilde{\bfT}}
\newcommand{\vr} {\tilde{u}{}^{\eps}}
\newcommand{\bftr} {\tilde{\bft}{}^{\eps}}
%\newcommand{\bu} {p}
\newcommand{\bp} {\boldsymbol{p}}
\newcommand{\bfu} {u}
\newcommand{\bfv} {\boldsymbol{v}}
\newcommand{\bd} {\boldsymbol{d}}
\newcommand{\bI} {\boldsymbol{I}}
\newcommand{\bfA} {\boldsymbol{A}}
\newcommand{\bfU} {\boldsymbol{U}}
\newcommand{\bfV} {\boldsymbol{V}}
\newcommand{\bfUt} {\dd{\bfU}}
\newcommand{\bfF} {\boldsymbol{F}}
\newcommand{\AS}{\mbox{\boldmath $\Acal$}}
\newcommand{\US}{\mbox{\boldmath $\Ucal$}}
\newcommand{\bxo} {\bfx\Zsup}
\newcommand{\ro} {r\zsub}
\newcommand{\bzzo} {\boldsymbol{z}\Zsup}
\newcommand{\bxx} {\bzet^{x}}
\newcommand{\rZ} {r\Zsup}
\newcommand{\sym}{^{\text{sym}}}
\newcommand{\bfuo} {\bfu\obs}
\newcommand{\tpe}{\tilde{p}^{\eps}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tq}{\tilde{q}}
\newcommand{\pe}{p^{\eps}}
%\newcommand{\pff}{\boldsymbol{u}^{\textit{i}}}
\newcommand{\pff}{\btu}
\newcommand{\qf}{q^{\mbox{\tiny{F}}}}
\newcommand{\po} {u\obs}
\newcommand{\ptr} {p^{\text{true}}}
\newcommand{\bfvo} {\bfv\obs}
\newcommand{\bfsigt} {\dd{\bfsig}}
\newcommand{\bfSigt} {\dd{\bfSig}}
\newcommand{\bksi} {\boldsymbol{\xi}}
\newcommand{\bzet} {\boldsymbol{\zeta}}
\newcommand{\betta} {\boldsymbol{\eta}}
\newcommand{\bksib}{\bar{\boldsymbol{\xi}}}
\newcommand{\xib}{\bar{\xi}}
\newcommand{\kb}{\bar{k}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfxb}{\bar{\bfx}} 
\newcommand{\bfxib}{\bar{\bfxi}}
\newcommand{\xb} {\bar{x}}
\newcommand{\bfW} {\boldsymbol{W}}
\newcommand{\bfeps}{\boldsymbol{\varepsilon}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\bfsig}{\boldsymbol{\sigma}}
\newcommand{\bfSig}{\boldsymbol{\Sigma}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathrsfs{B}}
\newcommand{\Jcal}{J}
\newcommand{\JCal}{\Jcal_{\!f}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ocal}{\mathfrak{O}}
\newcommand{\Tcal}{{\sf T}}
\newcommand{\TCal}{\Tcal_{\!f}}
\newcommand{\TCalo}{\Tcal_{\!f\!\text{,\tiny opt}}}
\newcommand{\TCalom}{\Tcal_{\!f\!\text{,\tiny opt}}^{\text{\tiny min}}}
\newcommand{\Ucal}{\mathcal{U}}

\newcommand{\ropm}{r\one^{\mbox{\tiny{$\pm$}}}}
\newcommand{\rtp}{r\two^{\mbox{\tiny{$+$}}}}
\newcommand{\rtm}{r\two^{\mbox{\tiny{$-$}}}}

\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}

\newcommand{\Scal}{\mathrsfs{S}}
\newcommand{\dip} {\! :\!}
\newcommand{\sip} {\!\cdot\!}
\newcommand{\derp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\oo} {\omega}
\newcommand{\OOr}{\OO^{-}_{\eps}}
\newcommand{\OO}{\Omega}
\newcommand{\OOm}{\Omega^{-}}
\newcommand{\OOc}{\Omega_{c}}
%\newcommand{\OOd}{\Omega_{\bd}}
\newcommand{\OOd}{{\Omega}}
\newcommand{\So}{S\obs}
\newcommand{\Sos}{\Gamma\obs_{\!\Sigma}}
\newcommand{\Soo}{\Gamma\obs_{\!\Omega}}
\newcommand{\OOt}{\Omega\true}
\newcommand{\G}{\Gamma}
\newcommand{\Gt}{\G\true}
\newcommand{\bfuG}{\bfu^{c}}
\newcommand{\bftG}{\bft^{c}}
\newcommand{\uG}{u^{c}}
\newcommand{\tG}{t^{c}}
\newcommand{\bfur}{p^{\eps}}
\newcommand{\bfsigr}{\bfsig^{\eps}}
\newcommand{\bfvr}{\tilde{\bfu}{}^{\eps}}
\newcommand{\bfvrS}{\bfvr_{\SN}}
\newcommand{\bftrS}{\bftr_{\SD}}
\newcommand{\bfvrG}{\bfvr_{\Gr}}
\newcommand{\bfut} {\dd{\bfu}}
\newcommand{\bfvt} {\tilde{\bfv}}
\newcommand{\bfutr} {\bfut{}^{\eps}}
\newcommand{\bfvtr} {\bfvt{}^{\eps}}
\newcommand{\bfpt} {\dd{\bfp}}
\newcommand{\bftt} {\dd{\bft}}
\newcommand{\Sigt} {\dd{\Sigma}}
\newcommand{\sigt} {\dd{\sigma}}
\newcommand{\tilU} {\dd{U}}
\newcommand{\tilu} {\dd{u}}
\newcommand{\tilp} {\dd{p}}
\newcommand{\herg}{\mathcal{H}}

\newcommand{\dGG}{\;\text{d}\G}
\newcommand{\dthxi}{\;\text{d}\vartheta_{\xib}}
\newcommand{\dVxi}{\;\text{d}V_{\xib}}
\newcommand{\dOO}{\;\text{d}\OO}
\newcommand{\iS}{\int_{\Scal}}
\newcommand{\Br} {B_{\eps}}
\newcommand{\Sr} {S_{\eps}}
\newcommand{\Gr} {\G_{\eps}}
\newcommand{\Brb} {\overline{B_{\eps}}}
\newcommand{\iBr} {\int_{\Br}}
\newcommand{\iGr} {\int_{\Gr}}

\newcommand{\sd}{\Sigma_{\text{\tiny D}}}
\newcommand{\sn}{\Sigma_{\text{\tiny N}}}

\newcommand{\Bi}{\mathcal{B}_1}
\newcommand{\Bo}{\mathcal{B}_2}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\bzero}{\boldsymbol{0}}

\newcommand{\bu} {\boldsymbol{u}}
\newcommand{\tbu} {\tilde{\boldsymbol{u}}}
\newcommand{\bt} {{\boldsymbol{t}}}
\newcommand{\btf} {{\boldsymbol{t}_f}}
\newcommand{\bbu} {\llbracket {\tbu}\rrbracket}
\newcommand{\bv} {\boldsymbol{v}}
\newcommand{\bff} {\boldsymbol{f}}
\newcommand{\Ga}{\G_{\mbox{\tiny{trial}}}}
\newcommand{\bxi} {\boldsymbol{\xi}}
\newcommand{\bxio} {\bxi\Zsup}
\newcommand{\tbv} {\tilde{\boldsymbol{v}}}
\newcommand{\Geps}{\Gamma_{\!\varepsilon}}
\newcommand{\bbb} {\llbracket\bar{\boldsymbol{v}}\rrbracket}
\newcommand{\bbv} {\llbracket {\tbv}\rrbracket}
\newcommand{\dbV} {\llbracket {V}\rrbracket}
\newcommand{\dbVe} {\llbracket {V_e}\rrbracket}
\newcommand{\dbVes} {\llbracket {V_{\nxs e^{\nxs*}}} \! \rrbracket}
\newcommand{\dbbV} {\llbracket {\boldsymbol{V}}\rrbracket}
\newcommand{\dbv} {\llbracket {\bv}\rrbracket}
\newcommand{\dbvz} {\llbracket {\bv_{\!\circ}}\rrbracket}
\newcommand{\dbvk} {\llbracket {\bv_\kappa}\rrbracket}
\newcommand{\dbva} {\llbracket {\bv_\alpha}\rrbracket}
\newcommand{\dbvap} {\llbracket {\bv_{\alpha+1}}\rrbracket}
\newcommand{\dbvd} {\llbracket {\dot\bv}\rrbracket}
\newcommand{\dbhv} {\llbracket \hat{\boldsymbol{v}}\rrbracket}
\newcommand{\btv} {\text{\bf{v}}}
\newcommand{\btu} {\text{\bf{u}}}
\newcommand{\btw} {\text{\bf{w}}}
\newcommand{\bw} {\boldsymbol{w}}
\newcommand{\bthh} {\hat{\boldsymbol{\theta}}}
\newcommand{\bphh} {\hat{\boldsymbol{\phi}}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bP} {\boldsymbol{P}}

\renewcommand{\Bo}{{B_R}}
\newcommand{\dualBR}[2]{\left< #1, #2 \right>_{\partial B_R}}
\newcommand{\dualGA}[2]{\left< #1, #2 \right>_{\Gamma}}
\newcommand{\bphi}{{\boldsymbol{\varphi}}}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
